Attentive Sequence to Sequence Translation for Localizing Clips of Interest by Natural Language Descriptions

We propose a novel attentive sequence to sequence translator (ASST) for clip localization in videos by natural language descriptions. We make two contributions. First, we propose a bi-directional Recurrent Neural Network (RNN) with a finely calibrated vision-language attentive mechanism to comprehensively understand the free-formed natural language descriptions. The RNN parses natural language descriptions in two directions, and the attentive model attends every meaningful word or phrase to each frame, thereby resulting in a more detailed understanding of video content and description semantics. Second, we design a hierarchical architecture for the network to jointly model language descriptions and video content. Given a video-description pair, the network generates a matrix representation, i.e., a sequence of vectors. Each vector in the matrix represents a video frame conditioned by the description. The 2D representation not only preserves the temporal dependencies of frames but also provides an effective way to perform frame-level video-language matching. The hierarchical architecture exploits video content with multiple granularities, ranging from subtle details to global context. Integration of the multiple granularities yields a robust representation for multi-level video-language abstraction. We validate the effectiveness of our ASST on two large-scale datasets. Our ASST outperforms the state-of-the-art by $4.28\%$ in Rank$@1$ on the DiDeMo dataset. On the Charades-STA dataset, we significantly improve the state-of-the-art by $13.41\%$ in Rank$@1,IoU=0.5$.

==> expr.tex <==
\section{Experiments}
\subsection{Datasets}
%We use DiDeMo~\cite{Hendricks_2017_ICCV} dataset for natural language video clip localization task. To verify the effectiveness of our standalone video subnet, We use THUMOS 14~\cite{THUMOS14} as our benchmark dataset for action detection task.
We use the DiDeMo~\cite{Hendricks_2017_ICCV} dataset for natural language video clip localization.
To verify the effectiveness of our standalone video subnet, We use THUMOS 14~\cite{THUMOS14} as our benchmark dataset for action detection task.

\noindent{\textbf{THUMOS 14}}.
THUMOS 14 is an action recognition and detection dataset. There are $101$ classes for action recognition task and $20$ classes for detection task. For action detection task, usually untrimmed videos from validation set and testing set are used as training data and testing data. There are $1,010$ videos in the validation set and $1,574$ in the testing set respectively. Only $200$ and $213$ videos in these two sets contain annotations within the $20$ action classes. Most recent literatures use these $413$ videos only for training and evaluation.
%We use both settings in our experiments. \ie, $1,010$ training videos with $1,574$ testing videos and $200$ training videos with $213$ testing videos.
In our experiments, we use these $413$ videos following most recent literatures.
The metric for THUMOS 14 dataset action detection task is $mAP$ (mean average precision) on different $IoU$s (Intersection over Union).
%The IoU thresholds are $0.1$, $0.2$, $0.3$, $0.4$ and $0.5$.
$mAP@IoU~0.5$ is usually used in recent papers.



\noindent{\textbf{DiDeMo}}.
DiDeMo is a dataset for natural language description localization in open-world videos. There are $33,005$, $4,180$ and $4,021$ video-description pairs in the training, validation and testing subsets respectively. 
To annotate video clips, DiDeMo segments videos every $5$ seconds. And the max available video length in this dataset is $30$ seconds. The ground truth of each video-description pair is annotated by multiple people on these segments. Therefor for each video, there are $21$ possible clips.
%Since annotations divide videos every $5$ seconds and max available video length is $30$ seconds, there are $21$ possible clips.
As we described previously, we address this task as a $21$-way classification task.
Following~\cite{Hendricks_2017_ICCV}, we use $Rank@1$, $Rank@5$ and $mIoU$ (mean Intersection over Union) as the evaluation metric. 
% MORE NEEDED?

\begin{comment}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
%\hline
%\multicolumn{8}{c}{Performances on THUMOS14, mAP@IoU $\alpha$} \\
\hline
Method & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 \\
\hline\hline
%Oneata~\etal~\cite{oneata2014lear}* & 36.58 & 33.60 & 27.00 & 20.76 & 14.37 & - & - \\
Oneata~\etal~\cite{oneata2014lear}* & $36.6$ & $33.6$ & $27.0$ & $20.8$ & $14.4$ & $-$ & $-$ \\
Yeung~\etal~\cite{yeung2016end}* & $48.9$ & $44.0$ & $36.0$ & $26.4$ & $17.1$ & $-$ & $-$ \\
Yuan~\etal~\cite{Yuan_2016_CVPR}* & $51.4$ & $42.6$ & $33.6$ & $26.1$ & $18.8$ & $-$ & $-$ \\
Yuan~\etal\cite{Yuan_2017_CVPR}* & $51.0$ & $45.2$ & $36.5$ & $27.8$ & $17.8$ & $-$ & $-$ \\
\hline
%Ours* & $49.0$ & $\mathbf{48.4}$ & $\mathbf{47.3}$ & $\mathbf{44.7}$ & $\mathbf{40.2}$ & $\mathbf{33.9}$ & $\mathbf{25.0}$ \\
%0.4958	0.4912	0.4729	0.4511	0.409	0.3368	0.2422
%Ours* ($200$ training videos) & $49.6$ & $47.3$ & $47.3$ & $45.1$ & $40.9$ & $33.7$ & $24.2$ \\
%0.5257	0.5212	0.5022	0.476	0.4326	0.3537	0.2567
%Ours* ($1,010$ training videos) & $\mathbf{52.6}$ & $\mathbf{52.1}$ & $\mathbf{50.2}$ & $\mathbf{47.6}$ & $\mathbf{43.3}$ & $\mathbf{35.4}$ & $\mathbf{25.7}$ \\
%Ours* & $\mathbf{52.6}$ & $\mathbf{52.1}$ & $\mathbf{50.2}$ & $\mathbf{47.6}$ & $\mathbf{43.3}$ & $\mathbf{35.4}$ & $\mathbf{25.7}$ \\
%0.527182	0.521462	0.502896	0.474858	0.422443	0.335378	0.234887
Ours* & $\mathbf{52.7}$ & $\mathbf{52.1}$ & $\mathbf{50.3}$ & $\mathbf{47.5}$ & $\mathbf{42.2}$ & $\mathbf{33.5}$ & $\mathbf{23.5}$ \\

\hline\hline
Richard~\etal~\cite{Richard_2016_CVPR} & $39.7$ & $35.7$ & $30.0$ & $23.2$ & $15.2$ & $-$ & $-$ \\
Shou~\etal~\cite{Shou_2016_CVPR} & $47.7$ & $43.5$ & $36.3$ & $28.7$ & $19.0$ & $10.3$ & $5.3$ \\
Shou~\etal~\cite{cdc_shou_cvpr17} & $-$ & $-$ & $40.1$ & $29.4$ & $23.3$ & $13.1$ & $7.9$ \\
Lin~\etal~\cite{Lin:2017:SST:3123266.3123343} & $50.1$ & $47.8$ & $43.0$ & $35.0$ & $24.6$ & $-$ & $-$ \\
Dai~\etal~\cite{Dai_2017_ICCV} & $-$ & $-$ & $-$ & $33.3$ & $25.6$ & $15.9$ & $9.0$ \\
Gao~\etal~\cite{Gao_2017_ICCV} & $54.0$ & $50.9$ & $44.1$ & $34.9$ & $25.6$ & $-$ & $-$ \\
Xu~\etal~\cite{Xu_2017_ICCV} & $54.5$ & $51.5$ & $44.8$ & $35.6$ & $28.9$ & $-$ & $-$ \\
Zhao~\etal~\cite{Zhao_2017_ICCV} & $\mathbf{66.0}$ & $\mathbf{59.4}$ & $51.9$ & $41.0$ & $29.8$ & $19.6$ & $10.7$ \\
\hline
%Ours & 56.29 & 55.55 & \textbf{53.94} & \textbf{50.41} & \textbf{44.95} & \textbf{37.49} & \textbf{27.35} \\
%Ours & $56.3$ & $55.6$ & $\mathbf{53.9}$ & $\mathbf{50.4}$ & $\mathbf{45.0}$ & $\mathbf{37.5}$ & $\mathbf{27.4}$ \\
%0.5665	0.5575	0.5335	0.51	0.4555	0.3687	0.2612
%Ours ($200$ training videos) & $56.7$ & $55.8$ & $\mathbf{53.4}$ & $\mathbf{51.0}$ & $\mathbf{45.6}$ & $\mathbf{36.9}$ & $\mathbf{26.1}$ \\ % 5e-3 mOHEM 20000 old test
%Ours & $56.7$ & $55.8$ & $\mathbf{53.4}$ & $\mathbf{51.0}$ & $\mathbf{45.6}$ & $\mathbf{36.9}$ & $\mathbf{26.1}$ \\
%0.57044	0.565223	0.539125	0.502734	0.439835	0.353739	0.236448
%Ours & $57.0$ & $56.5$ & $\mathbf{53.9}$ & $\mathbf{50.3}$ & $\mathbf{44.0}$ & $\mathbf{35.4}$ & $\mathbf{23.6}$ \\ % 5e-3 mOHEM 20000
%0.577673	0.571917	0.553698	0.513192	0.448076	0.350251	0.225191
%Ours & $57.8$ & $57.2$ & $\mathbf{55.4}$ & $\mathbf{51.3}$ & $\mathbf{44.8}$ & $\mathbf{35.0}$ & $\mathbf{22.5}$ \\ % 5e-3 rOHEM 15000
%0.580376	0.569213	0.543361	0.502338	0.447252	0.36089	0.230125
Ours & $58.0$ & $56.9$ & $\mathbf{54.3}$ & $\mathbf{50.2}$ & $\mathbf{44.7}$ & $\mathbf{36.1}$ & $\mathbf{23.0}$ \\ % 5e-3 mOHEM 13000


%\hline
%0.5516	0.5466	0.5268	0.4974	0.4496	0.3654	0.2642
%Ours ($1,010$ training videos) & $55.2$ & $54.7$ & $52.7$ & $49.7$ & $45.0$ & $36.5$ & $26.4$ \\
\hline
\end{tabular}
\end{center}
\caption{Action detection results on THUMOS 14 dataset (in percentage). The $IoU$ threshold used in evaluation varies from $0.1$ to $0.7$. - indicates that the results in corresponding papers are unavailable. * indicates that the results are generated on full testing set of $1,574$ videos.}
\label{tab:THUMOS14}
\end{table*}
\end{comment}


\subsection{Implementation Details}
We implement our ASST by TensorFlow~\cite{abadi2016tensorflow}.
We will make our code publicly available upon acceptance.

%During training time, we use Stochastic Gradient Descent (SGD) with Momentum $0.9$ as our optimizer. 
% ADAM ???
In our experiments, we build our ASST with two bi-directional LSTM layers for language subnet, four dilation layers, six squeezing layers and six expansion layers for video subnet. Our language subnet and video subnet take GloVe word embeddings~\cite{pennington2014glove} and two-stream ConvNets~\cite{simonyan2014two} feature as inputs.
Two-stream ConvNets consist of RGB network and optical flow network, which take original RGB images and optical flows as inputs, recognize static objects and motions in videos respectively. The channel size of LSTM states, dilation layers and squeezing-expansion layers are $512$, $1,024$ and $512$.
We use different training strategies for two tasks.

For action detection task, we use Inception-BN trained on ImageNet training set as our RGB network, and Inception-BN trained on UCF101~\cite{UCF101} split $1$ training set~\cite{wang2016temporal} as our optical flow network. We apply range dropout with rate $0.4$ on input feature.
We use mOHEM to select targets to be optimized in each iteration.
%Online Hard Example Mining (OHEM)~\cite{shrivastava2016training} to select training targets in each batch.
Any sampled clip with $IoU$ greater than $0.5$ with any annotation is considered as a positive example.
%The training targets are selected by mOHEM.
We use Stochastic Gradient Descent (SGD) with momentum $0.9$ as our optimizer. The learning rate starts from $5\times 10^{-3}$ and multiplies $0.9$ every $1,000$ steps. The model samples $5$ frames per second. At training time, we randomly stretch or compress our model by a scale within $[0.8, 1.25]$, then sample a clip of random time from training videos.
During inference, we slide our model along every testing video.
Non Maximum Suppression (NMS) with threshold $0.3$ within same class is applied as post processing.
% STEP 9?



For natural language localization in videos, we use Inception-V4~\cite{szegedy2017inception} trained on ImageNet~\cite{russakovsky2015imagenet} training set as our RGB network and Inception-BN~\cite{ioffe2015batch} trained on ActivityNet~\cite{caba2015activitynet} training set~\cite{xiong2016cuhk} as our optical flow network.
%We apply dropout on input visual feature with rate $[0.5, 1]$, context layers and LSTM with rate $[0.8, 1]$.
We apply range dropout on input visual feature with rate $0.5$, dilation layers and LSTMs with rate $0.8$.
We use Adam~\cite{kingma2014adam} as our optimizer. The learning rate starts from $5\times 10^{-4}$, and multiplies $0.9$ every $2,500$ steps.
%The frame sample rate are adjusted automatically.
The frame sample rate is $\frac{128}{30}$, so that our ASST can observe entire $30$-second video in one observation. We randomly move our network by random time deviation within $[-0.2, 0.2]$ seconds as data augmentation.
There are more than one annotation for each video-description pair. We first filter out annotations which has no overlap with other annotations of the same pair. Then, we randomly choose one annotation from remaining annotations for each iteration. To stabilize prediction, we average predictions from multiple model checkpoints.





\subsection{Experimental results}
\subsubsection{Action detection}



We first evaluate our video subnet for action detection task on THUMOS 14 dataset. We show our action detection performances on THUMOS 14 dataset in Table~\ref{tab:THUMOS14}.
%Some of recent literatures also showed their results at $IoU$ $0.6$ and $0.7$. We also show our results at $IoU$ $0.6$ and $0.7$ for a full comparison.
%We report our results at $IoU$ $0.3$ to $0.7$ due to limit of space.
We report our results at $IoU$ $0.3$ to $0.7$ following Shou~\etal\cite{cdc_shou_cvpr17}.

\begin{table}[ht]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|}
%\hline
%\multicolumn{8}{c}{Performances on THUMOS14, mAP@IoU $\alpha$} \\
\hline
Method & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 \\
\hline\hline
Richard~\etal~\cite{Richard_2016_CVPR} & $30.0$ & $23.2$ & $15.2$ & $-$ & $-$ \\
Shou~\etal~\cite{Shou_2016_CVPR} & $36.3$ & $28.7$ & $19.0$ & $10.3$ & $5.3$ \\
Shou~\etal~\cite{cdc_shou_cvpr17} & $40.1$ & $29.4$ & $23.3$ & $13.1$ & $7.9$ \\
Lin~\etal~\cite{Lin:2017:SST:3123266.3123343} & $43.0$ & $35.0$ & $24.6$ & $-$ & $-$ \\
Dai~\etal~\cite{Dai_2017_ICCV} & $-$ & $33.3$ & $25.6$ & $15.9$ & $9.0$ \\
Gao~\etal~\cite{Gao_2017_ICCV} & $44.1$ & $34.9$ & $25.6$ & $-$ & $-$ \\
Xu~\etal~\cite{Xu_2017_ICCV} & $44.8$ & $35.6$ & $28.9$ & $-$ & $-$ \\
Zhao~\etal~\cite{Zhao_2017_ICCV} & $51.9$ & $41.0$ & $29.8$ & $19.6$ & $10.7$ \\

\hline
%Ours & 56.29 & 55.55 & \textbf{53.94} & \textbf{50.41} & \textbf{44.95} & \textbf{37.49} & \textbf{27.35} \\
%Ours & $56.3$ & $55.6$ & $\mathbf{53.9}$ & $\mathbf{50.4}$ & $\mathbf{45.0}$ & $\mathbf{37.5}$ & $\mathbf{27.4}$ \\
%0.5665	0.5575	0.5335	0.51	0.4555	0.3687	0.2612
%Ours ($200$ training videos) & $56.7$ & $55.8$ & $\mathbf{53.4}$ & $\mathbf{51.0}$ & $\mathbf{45.6}$ & $\mathbf{36.9}$ & $\mathbf{26.1}$ \\ % 5e-3 mOHEM 20000 old test
%Ours & $56.7$ & $55.8$ & $\mathbf{53.4}$ & $\mathbf{51.0}$ & $\mathbf{45.6}$ & $\mathbf{36.9}$ & $\mathbf{26.1}$ \\
%0.57044	0.565223	0.539125	0.502734	0.439835	0.353739	0.236448
%Ours & $57.0$ & $56.5$ & $\mathbf{53.9}$ & $\mathbf{50.3}$ & $\mathbf{44.0}$ & $\mathbf{35.4}$ & $\mathbf{23.6}$ \\ % 5e-3 mOHEM 20000
%0.577673	0.571917	0.553698	0.513192	0.448076	0.350251	0.225191
%Ours & $57.8$ & $57.2$ & $\mathbf{55.4}$ & $\mathbf{51.3}$ & $\mathbf{44.8}$ & $\mathbf{35.0}$ & $\mathbf{22.5}$ \\ % 5e-3 rOHEM 15000
%0.580376	0.569213	0.543361	0.502338	0.447252	0.36089	0.230125
%Ours & $58.0$ & $56.9$ & $\mathbf{54.3}$ & $\mathbf{50.2}$ & $\mathbf{44.7}$ & $\mathbf{36.1}$ & $\mathbf{23.0}$ \\ % 5e-3 mOHEM 13000
%Ours & $\mathbf{54.3}$ & $\mathbf{50.2}$ & $\mathbf{44.7}$ & $\mathbf{36.1}$ & $\mathbf{23.0}$ \\ % 5e-3 mOHEM 13000
%0.576878	0.56941	0.547648	0.505152	0.450518	0.360867	0.233621
Ours & $\mathbf{54.8}$ & $\mathbf{50.5}$ & $\mathbf{45.1}$ & $\mathbf{36.1}$ & $\mathbf{23.4}$ \\ % 5e-3 mOHEM 11000


\hline
\end{tabular}
\end{center}
\caption{Action detection results on THUMOS 14 dataset (in percentage). The $IoU$ threshold used in evaluation varies from $0.3$ to $0.7$. - indicates the results in corresponding papers are unavailable.}
\label{tab:THUMOS14}
\end{table}

The most frequently used metric in recent papers for action detection is $mAP@IoU~0.5$. Our model  outperforms state-of-the-art methods by a notable margin of $15.3\%$.
Zhao~\etal~\cite{Zhao_2017_ICCV} achieved a good performance among all recent methods by building a hard coded context region. Our ASST's video subnet encodes video temporal context via multiple convolutional layers, which learns deep contextual temporal structure with multiple granularities, and is more capable of capturing video content at different scales, thereby achieving a much better performance.  

%the video context information are already encoded into the model implicitly. 
%Zhao~\etal achieved a superior performance at $IoU$ $0.1$ and $0.2$. But others $mAP$ decreases fast as $IoU$ increases, while ours decreases much slower.



%Comparing to other methods, 



%This is because our model makes more accurate predictions. We show our prediction in figure XXX.
% SHOW EXAMPLE?



% Our model can outperform most of recent results. Especially on larger $IoU$s, we can outperform state-of-the-art results by a large margin. 
% As IoU increases, our performance decreases slower than other methods. Which means, for predicted clips, our model is able to predict more accurate location estimation.


%Zhao~\etal~\cite{Zhao_2017_ICCV} used a sophisticated merging method, so we are unable to outperform them.

% The experimental results show that our visual subnet is good enough to encode video information.



%multiple steps analysis
%dropout vs range dropout



%Successes

%Failures
\begin{figure*}[t]
\begin{center}
\includegraphics[width=.95\linewidth]{result.pdf}
%\def\svgwidth{0.95\linewidth}
%\input{pic/Introduction.pdf_tex}
\end{center}
\caption{Visualization of our ASST's experimental results. The yellow bars above videos indicate ground truths. The bars under videos indicate our predictions. A green bar represents our prediction is correct. A blue bar represents our prediction overlaps with ground-truth annotation, but not accurate. A red bar represents our prediction does not overlap with ground truth. Best viewed in color.}
\label{fig:result}
\end{figure*}

\subsubsection{Natural language description localization}
We perform experiments on DiDeMo dataset for natural language description localization in videos. Table~\ref{tab:DiDeMo} shows our results and baselines provided in \cite{Hendricks_2017_ICCV}.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Method & Rank$@1$ & Rank$@5$ & $mIoU$ \\
\hline\hline
Frequency Prior~\cite{Hendricks_2017_ICCV} & $19.40$ & $66.38$ & $26.65$ \\
CCA~\cite{Hendricks_2017_ICCV} & $18.11$ & $52.11$ & $37.82$ \\
MCN~\cite{Hendricks_2017_ICCV} & $28.10$ & $78.21$ & $41.08$ \\
\hline
%Ours RGB & $25.64$ & $69.24$ & $39.30$ \\
%Ours Flow & $30.37$ & $73.54$ & $45.64$ \\
%Ours Two-stream & $30.64$ & $75.75$ & $45.95$ \\
Ours & $\mathbf{33.45}$ & $\mathbf{79.88}$ & $\mathbf{48.53}$ \\
\hline
\end{tabular}
\end{center}
\caption{Natural language localization in video results on test set.
%Our ASST outperforms all baselines on all metrics.
}
\label{tab:DiDeMo}
\end{table}

Our model outperforms MCN on all three metrics.
On Rank$@5$, our ASST is better than MCN by $1.67\%$.
On Rank$@1$ and $mIoU$, our ASST outperforms MCN significantly by $5.35\%$ and $7.45\%$ respectively.
In Figure~\ref{fig:result}, we show some of our localization results.
In the first example, our ASST successfully localized the sentence ``we can see someone in a mask'' and ``clerk hangs a blue shirt''.
For the third text query, ``a scary mask'', our ASST failed to generate an accurate prediction, but the predicted clip has an overlap with the ground-truth annotation.
One possible reason could be that ``a scary mask'' is an ambiguous description.
%In the second example, our ASST successfully localized ``baby begins to laugh''.
%For query ``babies left hand is touching its mouth'', our ASST predicted a clip that overlaps with the ground truth annotation, but not accurate. One reason could be that our model fails to focus on the word ``left''.
%For the third query ``baby puts hand in mouth while laughing'', Our predicted clip is visually similar to the query, but the baby is not touch its mouth.
%In the third example,
In the second example,
our ASST successfully detected ``the animal is eating the food'', but missed the first segment. In the first segment, the animal is eating with no food visible in its hands. Our ASST failed to localize ``animal is closest to camera'' and ``the animal approaches the cameraman aggressively''. Both descriptions are directly related to the camera (observer). Events related to the observer needed to be inferred from object and camera motion, which is hard to be modeled directly.
%The relation to the observer is difficult to model.

%TODO



%And we show successes and failures in figure XXX.

%Successes

%Failures

% Some analysis



\subsection{Ablation study}
We then perform ablation studies on the validation set from following three aspects: input visual modality, the importance of cross-modal local relevance and temporal endpoint feature. %In ablation studies, we use two-stream feature as input only.

\noindent{\textbf{Input visual modality}}.
% Single model
We first perform ablation study on how input visual modality influences our ASST's performance. We trained three models which take RGB, optical flow and concatenation of two-stream features as the input visual feature. The results are shown in Table~\ref{tab:Modal}.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Method & Rank$@1$ & Rank$@5$ & $mIoU$ \\
\hline\hline
%No language feature & $20.14$ & $66.10$ & $32.59$ \\
%\hline
RGB & $25.91$ & $73.11$ & $40.76$ \\
Flow & $29.38$ & $74.55$ & $45.09$ \\
Two-stream & $31.05$ & $76.58$ & $47.09$ \\
\hline
%No RNN context & $30.81$ & $76.41$ & $45.96$ \\
%Ours & $31.05$ & $76.58$ & $47.09$ \\
RGB + Flow & $31.12$ & $79.78$ & $46.30$ \\
\hline
Fusion & $\mathbf{33.47}$ & $\mathbf{81.77}$ & $\mathbf{49.08}$ \\
\hline
\end{tabular}
\end{center}
\caption{Ablations study on input visual modalities.}
\label{tab:Modal}
\end{table}

Within these three models, RGB model achieves inferior performance. The optical flow model outperforms RGB model significantly by more than $3.47\%$ on Rank$@1$. By concatenating both RGB and optical flow input feature, two-stream model further improves the optical flow model by $1.67\%$ on $mIoU$. The results show that both RGB and optical flow modality are important. Optical flow is still a good feature for video information modeling on tasks other than action recognition and detection. 

%Fusing
By feeding different input video data, our ASST learns relevance between natural language descriptions and video content from different aspects. Directly fusing RGB and optical flow models by a weight of $1:1.3$, the fused model achieves a similar performance on Rank$@1$, higher Rank$@5$ and lower $mIoU$ to single two-stream model. We then fuse all three models by a weight of $1:1.3:1.5$. The performance further improves around $2\%$ on all three metrics. The fusion weights are selected by ablation study. This fusion model is also our final model used for comparing with baselines.
In the following ablation studies, we use single two-stream model only.
%input modal
%RGB
%Flow
%Two-stream
%Fusion



\noindent{\textbf{Modeling cross-modal local relevance}}.
We perform ablation study to evaluate the necessity of early fusing natural language description and video content. We use plain video subnet as our baseline. This model contains no language information, learns localization prediction directly from video content. To evaluate the effectiveness of cross-modal deep fusion, we feed the language feature only once into video subnet via attention module. We choose three positions: final representation layer, last dilation layer and first dilation layer. The results are shown in Table~\ref{tab:Merge}.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Method & Rank$@1$ & Rank$@5$ & $mIoU$ \\
\hline\hline
No language feature & $20.14$ & $66.10$ & $32.59$ \\
\hline
Final representation layer & $26.67$ & $71.12$ & $41.99$ \\
%After context layers & $28.71$ & $75.43$ & $44.68$ \\
Last dilation layer & $29.69$ & $74.83$ & $45.14$ \\
First dilation layer & $29.64$ & $75.10$ & $45.26$ \\
%Before context layers & $29.81$ & $73.88$ & $46.02$ \\
\hline
%No RNN context & $30.81$ & $76.41$ & $45.96$ \\
%Ours & $31.05$ & $76.58$ & $47.09$ \\
Multiple feeding & $\mathbf{31.05}$ & $\mathbf{76.58}$ & $\mathbf{47.09}$ \\
\hline
\end{tabular}
\end{center}
\caption{Ablation study on modeling cross-modal local relevance.}
\label{tab:Merge}
\end{table}

In this table, the model that feeds language information on final representation layer achieves worst performance among all models with one-time language feature feeding. Feeding language on first dilation layer achieves a similar performance to feeding on last dilation layer with slightly better Rank$@5$ and $mIoU$.
Both models outperform the model that feeds language information on final representation layer significantly. Feeding language information multiple times achieves the best performance.
The results demonstrate the importance of modeling video-language local relevance. Feeding language feature on the final representation layer makes the model unable to build joint video-language hierarchies.
% just as we expected.

%we observe that earlier feeding achieves better performance. For earlier feeding, 


\begin{comment}

\subsubsection{The importance of language representation}
We first perform experiments to show the importance of language representation. We choose two baselines. The first baseline is our standalone visual subnet. This localization result depend on video only. The second baseline is encoding word feature without bi-directional RNN, which means there is no sentence-level context for word feature.

The results are shown in table~\ref{tab:Merge2}.




\subsubsection{Merging method of language feature}
In this part, we analyze different merging methods of language and video information. We test feed linguistic feature 

The results are shown in table~\ref{tab:Merge}.

%Position

%Method

\begin{table}[ht]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Method & Rank$@1$ & Rank$@5$ & mIoU \\
\hline
%Before Context Layers & $0$ & $0$ & $0$ \\
%First Context Layer & $0$ & $0$ & $0$ \\
%End of Context Layers & $0$ & $0$ & $0$ \\
%Final Representation Layer & $0$ & $0$ & $0$ \\
%\hline
Concat & $29.38$ & $75.41$ & $45.71$ \\
Adding & $29.90$ & $74.23$ & $46.08$ \\
Multiply & $31.05$ & $76.58$ & $47.09$ \\

\hline
\end{tabular}
\end{center}
\caption{Ablations study of merging method and position on validation set.}
\label{tab:Merge2}
\end{table}
\end{comment}

\noindent{\textbf{Temporal endpoint feature}}.
We also evaluate the effect of temporal endpoint feature (TEF) proposed by Hendricks~\etal~\cite{Hendricks_2017_ICCV}. The results are shown in Table~\ref{tab:TEF}.

\begin{table}[ht]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Method & Rank$@1$ & Rank$@5$ & $mIoU$ \\
\hline\hline
%MCN w/o TEF & $19.88$ & $62.39$ & $33.51$ \\
Ours w/o TEF & $30.07$ & $75.36$ & $45.89$ \\
%MCN & $27.57$ & $79.69$ & $41.70$ \\
Ours & $\mathbf{31.05}$ & $\mathbf{76.58}$ & $\mathbf{47.09}$ \\
\hline
\end{tabular}
\end{center}
\caption{Ablation study on temporal endpoint feature.}
\label{tab:TEF}
\end{table}

TEF improves MCN significantly by $38.68\%$ relatively on Rank$@1$. But TEF only improves our ASST by $3.26\%$ relatively. One reason could be that during the process of visual information encoding, every element in our final representation sequence has a large receptive field. The temporal position information is encoded implicitly.





==> model.tex <==
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=.95\linewidth]{network.pdf}
%\def\svgwidth{0.95\linewidth}
%\input{pic/network.pdf_tex}
\end{center}
\caption{An illustration of our model. Our model consists of an RNN-based language subnet (left) and a ConvNet-based video subnet (right).
    The two subnets are integrated via an attention module (top) on every dilation layer.
    In this example, the language subnet has two stacked LSTM layers. For the video subnet, there are three dilation layers, followed by three squeezing layers and three expansion layers.
    %Orange arrows represent convolution operations.
%representation layers.
The output of the last dilation layer is used as the input of first squeezing layer. Best viewed in color.}
\label{fig:network}
\vspace{-0.2cm}
\end{figure*}

\input{./related_works.tex}

\section{Our approach}
%\section{Attentive Sequence to Sequence Translation}
As illustrated in Figure~\ref{fig:network},
the proposed attentive sequence to sequence translator (ASST) consists of 
three
%two?
components: a video subnet for modeling video content, a language subnet for modeling natural language description and a multi-stage cross-modal attention module.
%Our ASST is end-to-end trainable.
%These two subnets are combined into one end-to-end model by a multi-stage attention module.

\subsection{Video subnet}
Our video subnet is shown on the right part in Figure~\ref{fig:network}.
First, the video subnet translates the input visual feature sequence into a representation sequence.
The length of the representation sequence and the length of the input feature sequence are identical.
Each element in this final representation sequence contains temporal visual contextual information, ranging from subtle details to global context, as well as clues from natural language descriptions.
Then, video clip representations are obtained by directly sampling clips on the final representation sequence.
%The base network consists of context layers and representation layers.
%On the last stage,
%we build different detection anchor groups on the final representation sequence for different tasks. 
%we directly sample clips on the final representation sequence depend on the task we are handling.
%We demonstrate our video subnet from these two aspects.

\subsubsection{Visual feature learning}
The video subnet is a 1D fully-convolutional network spanned on temporal domain.
We take a sequence of vectors $\{\mathbf{x}_{0}, \mathbf{x}_{1}, ..., \mathbf{x}_{t-1}\}$ with dimension $n_f$ as the input of the video subnet,
where $t$ is the number of elements in the input sequence, 
%sequence length of input visual feature.
We note the temporal length in seconds of the input sequence
%spanned on temporal domain
as $\tau$.
%\red{There are two process, One is xxx, the other is xxx. works together xxx}
%There are two processes.
%The subnet
Visual feature learning
consists of two stages.
One is attentive local temporal feature learning via stacked dilated convolution. The other one is global temporal context modeling via a squeezing-expansion process.
The video subnet transforms an input sequence $\{\mathbf{x}_{0}, \mathbf{x}_{1}, ..., \mathbf{x}_{t-1}\}$ to a representation sequence $\{\mathbf{x}'_{0}, \mathbf{x}'_{1}, ..., \mathbf{x}'_{t-1}\}$ via these two stages.
%with a same length as input sequence ${\mathbf{x}}$.

\noindent\textbf{Dilation Layers}. We first model the frame-level input features with their neighboring frames.
This process learns temporal hierarchical structure of the input sequence via stacked dilated convolution layers~\cite{kalchbrenner2016neural, Lea_2017_CVPR, oord2016wavenet, yu2015multi}.
%(\red{The context layer xxxxx, illustrate the usage.})
%We first feed the input visual feature sequence into 
%It is done by several dilated convolution layers~\cite{kalchbrenner2016neural, Lea_2017_CVPR, oord2016wavenet, yu2015multi} for temporal context learning.
The dilation rates are doubled from each layer forward.
Stacked dilated convolution increases receptive field in an exponential speed as the network goes deeper, while the size of feature maps remain unchanged.
These layers model temporal contextual structures at multiple time scales for every input frame.
%Natural language descriptions interact with visual information within context layers.
%We will demonstrate this part later. 
In Figure~\ref{fig:network}, we show a model with three dilation layers.
We additionally apply shortcut connections~\cite{he2016deep} between every two adjacent layers.
%by adding feature map before last dilated convolution to the next corresponding feature map.
Shortcut connections shorten the information path from the bottom to the top of the network, which makes the training process easier.
%\red{(how the shortcut connection works. directly pass the output to , the apply add. retain the information from bottom layer)}
%The shortcut connections are very helpful for model training.
After the above operations, every element in the last dilation layer perceives a large temporal window.
%and natural language information.
%However, context layers only models local contextual temporal structure of input sequence without global visual information, 
%there is still no global context from the entire video sequence, 
%while global context is vital for localizing clips in entire input video.

%linear? bilinear? interpolation
\noindent\textbf{Squeezing-expansion Layers}. %\red{(Representation layers encode global context. Please illustrate the benefit, why need this)}
The dilation layers demonstrated above contain only local temporal contextual structures.
The elements in the final dilation layer do not observe the entire input visual sequence.
However, global context is vital for localizing clips in videos.
For example, someone may be interested in localizing the clip when a certain target event happens the second time.
To distinguish the positive clip from visually similar negative clips, the model needs to understand the global context to make accurate predictions.
%what is current observed local visual information representing under the context of entire video.
To model global context information, we generate our final representation sequence through a squeezing phase followed by an expansion phase (Figure~\ref{fig:network}).
The output of the last dilation layer is used as the input of the first squeezing layer.
%The architecture of ``Representation Layers'' is similar to top-down module in object detection~\cite{lin2016feature, Lin_2017_ICCV, shrivastava2016beyond}. 
The architecture of ``Squeezing-Expansion Layers'' can be viewed as a 1D version of top-down module in object detection~\cite{lin2016feature, Lin_2017_ICCV, shrivastava2016beyond}.
%Though representation layers are built on context layers, there is no global representation in this process. %???
The model further encodes global context information into the final representation through this squeezing-expansion process.

The squeezing phase consists of several convolution layers with stride $2$ and kernel size $3$, and generates a global representation vector. This vector summarizes visual information and temporal structures across all the input visual features.
It will be used as global context background for further representation learning.
%\red{more details}

%\red{The expand phase expand the representation in a reverse order}
The expansion phase and the squeezing phase are connected by a convolution operation.
During the expansion phase, we expand the global representation vector in a reverse order as we did during the squeezing phase, until it reaches the size of the last dilation layer.
%Then we expand the global representation to each squeezed layer in a reverse order.
We apply a convolution with kernel size $1$ on each feature map from the squeezing phase, while the output is added to the expanded feature map with the same size.
The result feature map includes both global contextual information (from expanded feature map) and local contextual information (from convolved feature map in the squeezing phase).
We use linear interpolation as our expansion operation. 
The output of the last layer is our final representation sequence.

With dilation layers and squeezing-expansion layers, our translator is able to transform input visual sequence into a representation sequence, exploiting both global and local temporal contextual structures.

%\red{Another paragraph, with the context layer and the representation layer, our translator is able to xx, the representation xxx}

%a hierarchical structure for the network to jointly model language description and video content.

%During representation layers, the input features are first gradually squeezed into one global representation vector, then expanded to the size of each previous representation layers in a reverse order. Every representation layer in squeeze phase is passed through a convolution convolution layer with kernel size $1$ and added to corresponding layer in expansion phase. We use linear interpolation as our expansion operation. The last layer is our final representation sequence.

%\subsubsection{Detection anchor building}
\subsubsection{Clip sampling}
% CHANGE NAME TO ``clip sampler'' ?
% bilinear? linear? interpolation
% Possible regions / proposals are provided by dataset !!
We sample our 
%detection anchors
%clip samplers
target clips
on the final representation sequence $\{\mathbf{x}'\}$ by RoI-pooling~\cite{girshick2015fast} in temporal domain with linear interpolation.
For each clip sampler, we sample seven elements from the final representation sequence as the input.
%detection anchor

% IS THIS 'DILATED' NECESSARY?
%The detection anchor
The clip sampler is a $2$-layer convolutional network with kernel size $3$.
%, which means the input for each detection anchor is $7$
%All detection anchors
All clip samplers
share weights. We use different
clip sampling
%anchor building
strategies for different tasks.

For the natural language localization task, we address it as a classification problem by enumerating clip proposals. We build one
%anchor
sampler
for each possible clip. Each
%anchor
sampler generates one scalar, which represents the score for the corresponding video clip.
% SCORE?
We also feed TEF (temporal endpoint features) into
%anchors
clip samplers by concatenating TEF to every sampled vector
%detection anchors
following \cite{Hendricks_2017_ICCV}.
Finally, a softmax loss function is applied over all
clip samplers
%anchors
to train our ASST in a discriminative way.

% FIGURE FOR ANCHOR BUILDING?

For the action detection task, we build
%detection anchors
clip samplers similar to \cite{ren2015faster}.
%Except from natural language clip detection task, we can also build anchors for action detection.
We have six groups of
%anchors. 
samplers.
%The
% DISTINGUISH LENGTH AND TEMPORAL LENGTH
The $i$-th clip sampler group consists of clips with length $l_0^i=\frac{\tau}{2^{i}}$, where $0 \leq i \leq 5, i \in \mathbb{N}$, and $\tau$ is the temporal length of final representation sequence $\{\mathbf{x}'\}$.
The distance of every two adjacent samplers is $\frac{1}{4}l_0^i$. Therefore, there are $2^{i+2}-3$ samplers in the $i$-th group.
%anchor
%anchors
%anchors
%anchor
%These detection anchors share weights as well.
For each clip sampler, we predict class label $y$, center deviation $d_c$ and $\log$ difference from the default clip length $d_l$.
During inference, the temporal location of each clip sampler's prediction is calculated by,
%anchor
%of length 
%anchor
\begin{equation}
(\hat{c}, \hat{l}) = (c_{0}+d_{c}l_{0}, e^{d_l}l_{0})
\label{eq:boxPred}
\end{equation}
where $c_0$ is the center coordinate of the default window,
$l_0$ is the length of each clip,
$\hat{c}$ is the center coordinate of the predicted window and $\hat{l}$ is the length of the window.
We use standard $(n_c+1)$-class softmax loss, where $n_c$ is the number of classes.
Smooth-$L1$ loss is used to perform classification and temporal coordinate regression following most object detection literatures~\cite{dai2016r, Huang_2017_CVPR, Lin_2017_ICCV, liu2016ssd, ren2015faster}.
%\red{cite more papers}


\subsection{Language subnet}
%\subsubsection{Simple language}
%\subsubsection{RNN context}
The architecture of our language subnet is shown on the left part in Figure~\ref{fig:network}.
We use pre-trained word embeddings as word-level inputs.
Stacked bi-directional LSTM layers are built on top of word embeddings for sentence context modeling~\cite{wu2016google}. We also add shortcut connections from the input to the output of each LSTM layer for more efficient training.

We modify standard bi-directional LSTM by adding one convolution operation with kernel size $1$ after concatenating forward and backward output states. It is helpful for bi-directional LSTM's residual learning. We also apply a convolution operation with kernel size $1$ on the input word embeddings to adjust dimension for residual learning.

\begin{equation}
\begin{aligned}
\{\mathbf{w}_0^{i+1}, \mathbf{w}_1^{i+1}, ..., \mathbf{w}_{n-1}^{i+1}\} = &~ biRNN_i(\mathbf{w}_0^i, \mathbf{w}_1^i, ..., \mathbf{w}_{n-1}^i)\\
+ &~ \{\mathbf{w}_0^{i}, \mathbf{w}_1^{i}, ..., \mathbf{w}_{n-1}^{i}\},
\end{aligned}
\label{eq:birnn}
\end{equation}
where $n$ is the number of input words, $\{\mathbf{w}^i\}$ is the word-level feature sequence of the $i$-th layer
%\red{to add $w_n^{i}$}
We stack $p$ layers of bi-directional LSTM in our experiments.
The last output sequence $\{\mathbf{w}_0^{p}, \mathbf{w}_1^{p}, ..., \mathbf{w}_{n-1}^{p}\}$ is the output of the language subnet which will be used as the input of the cross-modal attention module.
%\red{CONV}

%GLU!!!
We choose Gated Linear Unit (GLU)~\cite{dauphin2016language} as the non-linearity function of convolutions for language modeling. GLU processes a input vector $[\mathbf{q}_0, \mathbf{q}_1]$ by,
\begin{equation}
GLU([\mathbf{q}_0, \mathbf{q}_1]) = \mathbf{q}_0 \odot \sigma(\mathbf{q}_1),
\end{equation}
where $\mathbf{q}_0$ and $\mathbf{q}_1$ are the inputs to the GLU with dimension $d$, $\sigma$ is the sigmoid function, and $\odot$ is element-wise multiplication.
GLU has been used in context modeling in natural language processing~\cite{dauphin2016language,gehring2017convolutional}. The gate $\sigma{\mathbf{q}_1}$ dynamically controls data flow via gating mechanism.
GLU shows superior performance than ReLU in our preliminary experiments.
%\red{GLU has been used in xxx, how does it work, what's the benifit.}
% GLU is better because of experiments?
% Conv?

\subsection{Cross-modal attention module}

\begin{figure}[t]
\begin{center}
\includegraphics[width=.95\columnwidth]{Attention.pdf}
%\def\svgwidth{0.95\columnwidth}
%\input{pic/Attention.pdf_tex}
\end{center}
\caption{An illustration of the attention module for combining the video subnet and the language subnet on one dilation layer.
    This module takes language feature (left) and video feature (bottom right) as inputs.
    It first generates an attention weight matrix from both input features, and then attends language feature for every video frame. This attended language feature multiplies with input video feature.
%works as a gate
%.
    After a convolution operation, shortcut connection is used to connect visual feature maps across adjacent dilated layers.    
%    cross dilated layers. \red{cross??}
Best viewed in color.}
\label{fig:Attention}
\end{figure}

To combine our video subnet and language subnet, we introduce a cross-modal attention module that combines visual and linguistic information.
%similar to the attention module proposed by Gehring~\etal~\cite{gehring2017convolutional}. 
This attention module is applied on every dilation layer.
Since different dilation layers aggregate temporal contextual information at
%different granularities
different temporal scales
, feeding language feature on every dilation layer enables our model exploits video-language relevance at multiple temporal scales.
%\red{rewrite}
In addition, the attention module attends word representations for each frame. It yields more detailed understanding of video content and description semantic.
%\red{rewrite}
In Figure~\ref{fig:Attention}, we show our attention module for one dilation layer. 

For each layer, the attention module takes language feature $\{\mathbf{w}_0, \mathbf{w}_1, ..., \mathbf{w}_{n-1}\}$ and visual feature $\{\mathbf{v}_0, \mathbf{v}_1, ..., \mathbf{v}_{m-1}\}$ as inputs.
We split language feature $\{\mathbf{w}_0, \mathbf{w}_1, ..., \mathbf{w}_{n-1}\}$ into two sequences by convolutions with kernel size $1$:
$\{\mathbf{w}_0^a, \mathbf{w}_1^a, ..., \mathbf{w}_{n-1}^a\}$ and $\{\mathbf{w}_0^v, \mathbf{w}_1^v, ..., \mathbf{w}_{n-1}^v\}$.
$\{\mathbf{w}^a\}$ is used for attention weight matrix computation. And $\{\mathbf{w}^v\}$ is used for further feature computation.
%\red{rewrite, how to get a and v}
We also compute $\{\mathbf{v}_0^a, \mathbf{v}_1^a, ..., \mathbf{v}_{m-1}^a\}$ a convolution from $\{\mathbf{v}\}$.
$\{\mathbf{v}^a\}$ is used as another input for attention weight computation. The attention weight matrix is computed as,
%\red{rewrite, v}
% \alpha or A ?
\begin{equation}
\begin{aligned}
A'_{ij} &= \frac{\mathbf{w}_i^a \cdot \mathbf{v}_j^a}{n_c},  \\
A_{ij} &= \frac{e^{A'_{ij}}}{\sum_i e^{A'_{ij}}},
\end{aligned}
\end{equation}
where $n_c$ is the dimension of $\mathbf{w}_i^a$ and $\mathbf{v}_j^a$, and $A$ is the attention weight matrix with size $n \times m$. We use this matrix to compute vision
%dependent
attended
language feature,
\begin{equation}
\mathbf{u}'_j = \sum_i A_{ij}\mathbf{w}_i^v.
\end{equation}

We then apply element-wise multiplication on $\{\mathbf{u}'\}$ and $\{\mathbf{v}\}$,
\begin{equation}
\mathbf{u}_j = \mathbf{u}'_j \odot \mathbf{v}_j.
\end{equation}

%$\{u\}'$ can be viewed as a generalized conditional normalization.
%$\{\mathbf{u}\}'$ can be viewed as a gate for visual context information from dilated convolution.

%CONDITIONAL NORMALIZATION?
%GATE

$\{\mathbf{u}\}$ is our language augmented context for this dilation layer.
We apply a BatchNorm~\cite{ioffe2015batch} followed by a ReLU to normalize the output.
%, same as other convolution layers.
%stabilize the model
Finally, we convolve $\{\mathbf{u}\}$ once and add it with the feature map before the last dilated convolution, as the input for the next dilated convolution.

%as our two branches of word representation from linguistic subnet. These two sequences are used for attention weight matrix computation and representation computation respectively. $\{\mathbf{w}_0^a, \mathbf{w}_1^a, ..., \mathbf{w}_{n-1}^a\}$ computes attention weight matrix with attention branch from visual subnet $\{\mathbf{v}_0^a, \mathbf{v}_1^a, ..., \mathbf{v}_{m-1}^a\}$ as:



%Similarly, we have two branches of vision feature: $\{\mathbf{v}_0^a, \mathbf{v}_1^a, ..., \mathbf{v}_{m-1}^a\}$ and $\{\mathbf{v}_0^v, \mathbf{v}_1^v, ..., \mathbf{v}_{m-1}^v\}$. The attention matrix is firstly computed as:

%Then we concatenate the output sequence $\{\mathbf{u}_0, \mathbf{u}_1, ..., \mathbf{u}_{n-1}\}$ and $\{\mathbf{v}_0^v, \mathbf{v}_1^v, ..., \mathbf{v}_{n-1}^v\}$ as a joint language-vision feature sequence. Finally, we apply one convolution layer on the joint feature sequence and add with previous layer as the output of this context layer. 



\subsection{Model Training}
%We use following training techniques to 
During our experiments, we find the following training techniques useful for our model training.

% ??? IS THIS NEW ???
\noindent{\textbf{Range Dropout}}.
In our experiments, we regularize our model by an improved version of dropout operation. We name it as ``Range Dropout''. For a regular dropout operation with rate $r$, any element in input tensor $X$ has a chance of $1-r$ to become $0$. $X$ is then scaled to $\frac{1}{r}$ to keep the expectation unchanged.

%The ``Range Dropout'' is based on the observation above. 
We propose to use a variable instead of a constant number as dropout rate.
We use a random real number within range $[r, 1]$ as our dropout rate. The rate varies in every iteration. With random dropout rate, models are able to observe more data with different variations but same expectation.

\noindent{\textbf{Mean Online Hard Example Mining}}.
%\red{rewrite anchors}
We use Online Hard Example Mining~\cite{shrivastava2016training} (OHEM) to select clip samples 
for 
%optimizing
gradient computation
in each batch for the action detection task. In our experiments, we select clip samples by a threshold 
based on statistics of all classification losses within a batch. For simplicity, we only use the mean
value computed on one batch as our threshold for this batch.
% generalized mean / power mean with exponent 1 and 2
%of mean value from all anchors' losses within a batch.
We name this mechanism as mOHEM (mean Online Hard Example Mining). 
mOHEM requires no hyper parameter.
%The only hyper parameter needed for mOHEM is the exponent $p$ for power mean computation.
Our mOHEM is able to dynamically focus on hard examples with large losses on different loss distributions.
% rOHEM ?
%We also explored different threshold for OHEM, like root of mean square. We name this mechanism as rOHEM (root-of-mean-square Online Hard Example Mining). For same distribution, RMS is larger than mean value. In our experiments, rOHEM achieves similar performance to mOHEM's.
%For example, a loss distribution with most of data have a small value, mOHEM will focus on data with large values only. 

% FOR UNBALANCED DISTRIBUTION

% NO HYPER PARAMETER NEEDED





==> related_works.tex <==
\section{Related work}
%\noindent{\textbf{Object detection}}.
%$Object detection is one of the fundamental tasks in computer vision.
%$Many deep learning based approaches have been proposed for this problem~\cite{dai2016r, Huang_2017_CVPR, Lin_2017_ICCV, liu2016ssd, ren2015faster}.
%$Currently, the general idea of state-of-the-art object detection models is to build detection anchors on the feature layers of the backbone network.
%$In some recent works, the top-down module has been proven useful for global context awareness~\cite{lin2016feature, Lin_2017_ICCV, shrivastava2016beyond}.
%$Global context from the entire video sequence can be vital for video clip understanding.
%$We thus incorporate a similar top-down module to learn global context.

\noindent{\textbf{Action detection in videos}}.
Action detection localizes interested video clips given action labels.
This task is usually divided into two branches: temporal detection and spatio-temporal detection.
For temporal detection~\cite{THUMOS14}, the model needs to output the start and end time of each action clip.
For spatio-temporal detection~\cite{pantofaru2017ava}, besides temporally localizing the actions, the model also generates the spatial locations of the actions for each frame.
%the spatial locations of target actions on each frame are also needed.
%We do not consider spatial localization in this paper.

% Temporal detection
Two-stream ConvNets~\cite{simonyan2014two, wang2015towards} and $3$D-ConvNets~\cite{tran2015learning} have been proposed to model video sequence data for action recognition. These methods have been widely used in temporal action detection~\cite{Lin:2017:SST:3123266.3123343, cdc_shou_cvpr17, Xu_2017_ICCV, Zhao_2017_ICCV}
and other video analysis tasks,~\eg,~video captioning~\cite{venugopalan15iccv}.
%\cite{Kalogeiton_2017_ICCV2, Kalogeiton_2017_ICCV, Sigurdsson_2017_ICCV}. % MORE CITATION?
Shou~\etal~\cite{cdc_shou_cvpr17} applied frame-level classification via a modified $3$D-ConvNet.
Lin~\etal~\cite{Lin:2017:SST:3123266.3123343} adopted Single-Shot-Detector~\cite{liu2016ssd} to detect interested actions in one shot.
Xu~\etal~\cite{Xu_2017_ICCV} tried to tackle the problem of temporal proposal generation. They incorporated an RoI-pooling layer followed by a classification branch and a temporal coordinate regression branch.
Zhao~\etal~\cite{Zhao_2017_ICCV} achieved a good performance by hard coding context regions, which enables the detector to model temporal context. They also proposed a sophisticated region merging strategy.
%\red{(Please add one sentence talking about our method,)}
We aggregate contextual temporal structures via dilated convolutional layers, followed by squeezing-expansion layers.
Our model jointly encodes neighboring and all observable visual information, which is more flexible for temporal structure modeling.

\noindent{\textbf{Natural language object localization}}.
Natural language object localization~\cite{hu2016natural, mao2016generation} is to localize objects of interest in images spatially by natural language descriptions.
%This is a similar task to the natural language localization in videos.
Mao~\etal~\cite{mao2016generation} encoded each possible region by an LSTM, and trained the model in a discriminative way by using a softmax loss over all encoded regions.
Hu~\etal~\cite{hu2016natural} ranked each object proposal by considering spatial configuration, local visual information and global visual information.
%Hu~\etal~\cite{hu2016natural} ranked each object proposal by scoring given natural language description conditioned by spatial configuration, local visual information and global visual information.
Rohrbach~\etal~\cite{rohrbach2016grounding} used attention mechanism to choose the region that could be best used for description reconstruction.
Nagaraja~\etal~\cite{nagaraja2016modeling} localized referred objects by understanding referring expressions via integrating context between objects.
In this paper, we focus on natural language video clip localization. We propose a novel ASST to jointly learn a video-language representation.


%VIDEO-LANGUAGE ALIGNMENT?

%CLEVR?

%VQA?

%\noindent{\textbf{Sequence to sequence learning}}.
%Sequence to sequence learning is a important research area in recent years, and being widely applied in many areas, \eg, machine translation and captioning \etc.
%Most work applies Recurrent Neural Network (RNN) to build encoder for parsing input sequence and decoder for generating output sequence~\cite{donahue2015long, sutskever2014sequence}. 
%Recently, Gehring~\etal~\cite{gehring2017convolutional} adopt Convolutional Neural Network (CNN) with attention module to build a convolutional sequence to sequence learning model. On each generation step, this model generates one element by hierarchically attending convolved input sequence and causal convolved previously generated output sequence.

%\noindent{\textbf{Multi-modal representation learning}}.
%Multi-modal representation learning is a research area about exploring relevance cross data modality, like image and natural language. Common cross-modal solutions is mapping cross-modal data independently into a unified semantic space, followed by distance measuring~\cite{frome2013devise}. These models are usually optimized by ranking loss or triplet loss. Karpathy~\etal~\cite{karpathy2015deep} apply bi-directional RNN for language modeling and R-CNN for image region modeling.

\noindent{\textbf{Video clip localization by natural language descriptions}}.
%\red{(It is a new task. MCN is proposed, it is a ranking based method)}
Video clip localization by natural language descriptions is a new task introduced by Hendricks~\etal~\cite{Hendricks_2017_ICCV}. Hendricks~\etal~\cite{Hendricks_2017_ICCV} proposed a Moment Context Network (MCN) to handle this task. MCN is a ranking based method. It embeds description and video clip information into a unified space individually, and ranks video clips by measuring distance between video clip embeddings and sentence embeddings. MCN considers representations from two modals separately, ignores detailed relevance between two modals.
Our ASST explores cross-modal relevance at finer granularities, which is able to better exploit detail information.

%CCA



%Classic multi-modal representation learning work for dealing with natural language and visual data are usually mapping them independently into a unified semantic space, Some recent work start to 

%Recurrent neural network based sequence to sequence learning~\cite{donahue2015long, sutskever2014sequence} and convolution based sequence to sequence learning~\cite{gehring2017convolutional} have shown good performances in many applications.  

%TODO

%Our model is a task dependent one-to-one video translation model. 


% In our network, we model our temporal video feature in a sequence to sequence learning style.

%Bijection
%one-to-one correspondence

